Cross-Lingual Ability of Multilingual BERT: An Empirical Study

Recent work has exhibited the surprising cross-lingual abilities of multilingual BERT (M-BERT) -- surprising since it is trained without any cross-lingual objective and with no aligned data. In this work, we provide a comprehensive study of the contribution of different components in M-BERT to its cross-lingual ability. We study the impact of linguistic properties of the languages, the architecture of the model, and the learning objectives. The experimental study is done in the context of three typologically different languages -- Spanish, Hindi, and Russian -- and using two conceptually different NLP tasks, textual entailment and named entity recognition. Among our key conclusions is the fact that the lexical overlap between languages plays a negligible role in the cross-lingual success, while the depth of the network is an integral part of it. All our models and implementations can be found on our project page: http://cogcomp.org/page/publication_view/900 .

==> Intrinsic.tex <==

\section{Intrinsic study: BERT vs Flair vs word2vec}
Compare enfake-en, enfake-es, enfake-hi, enfake-ru top-1 and top-3 results on XNLI parallel hypothesis. 



\begin{table*}[!htbp]
\centering
\begin{threeparttable}
\caption{Similarity between Parallel Sentences - Intrinsic Measure}
\begin{tabular}{ c c c c c c } 
\toprule
\textbf{Language-1} & \textbf{Language-2} & \textbf{Metric} & \textbf{BERT} & 
\textbf{Flair} & \textbf{Deep Word2Vec} \\
\midrule
\multirow{2}{*}{enfake} & \multirow{2}{*}{en} & Top-1 &  &  79.1 & 0.1 \\
 &  & Top-3 &  & 86.3& 0.6 \\
\midrule
\multirow{2}{*}{enfake} & \multirow{2}{*}{es} &  Top-1 & 46.6 & 2.0 & \\
 &  & Top-3  & 57.9 & 4.7 & \\
\midrule
\multirow{2}{*}{enfake} & \multirow{2}{*}{hi} & Top-1 & 17.4 &  0.1 \\
 &  & Top-3  &  26.0 & 0.8 \\
\midrule
\multirow{2}{*}{enfake} & \multirow{2}{*}{ru} & Top-1 & 41.3 & 1.6 & \\
 &  & Top-3 & 56.5 & 3.8 \\
\bottomrule
\end{tabular}
    \begin{tablenotes}
    \small
    \item 
    \end{tablenotes}
\end{threeparttable}
\label{tbl:Intrinsic}
\end{table*}


\section{Miscellaneous}

Premise in English and Hypothesis in target and vice versa.



==> Limitations.tex <==
\begin{itemize}
    \item In this work, we studied only cross-lingual ability of bilingual BERT instead of the multilingual BERT, where there could be more interaction among different languages.
    \item The definition of \textit{Structure of a Language} and \textit{Structural Similarity} is obscure (we tried to give intuitions about structure of language). 
    \item In Section~\ref{subsec:LanguageMarker}, we added language identity marker in only one way. Language identity could have been incorporated in many other ways. 
\end{itemize}









==> Notations.tex <==
For better understanding, throughout this paper, we use bilingual BERT (trained only on two languages) instead of multilingual BERT. We denote bilingual BERT trained on language A and B as A-B, e.g. BERT trained on English (en) and Hindi (hi) as en-hi, similarly for Spanish (es) and Russian (ru).

Unless otherwise specified, for English we use 1 GB sample from English Wikipedia text and for other languages, we use the entire Wikipedia text, we use 32 batch size, 1e-4 learning rate and 2 Million iterations for pre-training bilingual BERT. In section \ref{sec:LinguisticFeature} we introduce a new language called \textit{enfake} constructed from English, we use 1 GB sample for enfake also (unless specified).

\textsc{Cross-Lingual Learning:} Cross-lingual learning refers to a situation where a model is trained/fine-tuned using a labeled data in a source language (say English) and tested on a different target language (say Hindi). 

% \textbf{Cross-Lingual Similarity: } Similarity between vector representation of text in Language A and Language B.





























==> Notrequired.tex <==
% What are the components we are going to study
% Why they are important
From Section~\ref{sec:LinguisticFeature}, we observe that bilingual BERT recognizes the language structure effectively \sm{too strong}, while other models like bilingual word2vec/fasttext/flair couldn't (refer appendix). \sm{we can't refer to results that we haven't presented} We envisage that BERT potentially gains the ability to recognize language structure because of its deepness, a large number of parameters and multi-head self-attention (which none of the other models uses).

In this section, we study the contribution of different components of bilingual BERT architecture namely 
\begin{enumerate*}[label=(\roman*)]
    \item depth, 
    \item multi-head attention and,
    \item the total number of parameters. 
\end{enumerate*} The motivation is to understand which components are crucial for its cross-lingual ability.

We perform all our cross-lingual experiments on XNLI dataset with English as the source and Russian as the target language, we measure cross-lingual ability by the difference between the performance of English and Russian (lesser the difference better the cross-lingual ability).



\subsubsection{Depth}
% Write why do we think depth is important.

% Despite the cross-lingual ability of multilingual BERT, \cite{wu2019beto} shows that multilingual BERT retains the language identity, which is intuitive as identifying the language helps both NSP and MLM objective. However, retaining the language identity doesn't necessarily hurts cross-lingual performance as these features will be ignored when fine-tuned on supervised downstream task.

We presume the ability of multilingual BERT to extract good semantic and structural features is a crucial reason for its cross-lingual effectiveness and the deepness of multilingual BERT helps it extract good language features.   

In this section, we study the effect of depth on both the monolingual and cross-lingual performance of multilingual BERT.  We fix the number of attention heads and change the size of hidden units and intermediate units such that the total number of parameters are almost the same (size of intermediate units is always 4$\times$ size of hidden units) 

From Table~\ref{tbl:Depth}, we can see that deeper models not only perform better on English but are also better cross-lingual($\Delta$). We can also see a strong correlation between performance on English and cross-lingual ability ($\Delta$), which further supports our assumption that the ability to extract good semantic and structural features is a crucial reason for its cross-lingual effectiveness.

% \sm{I don't know what I'm looking at. Are these F1 scores? What is the parameters column? (millions of params?)}

\begin{table*}[!htbp]
\parbox{.45\linewidth}{
\small
\centering
\begin{threeparttable}
\caption{Model Architecture - Contribution of Depth}
\label{tbl:Depth}
\begin{tabular}{ c c c c c c} 
\toprule
\multicolumn{3}{c}{} & \multicolumn{3}{c}{\textbf{XNLI}} \\
\cmidrule{4-6}
\textbf{Parameters (in Millions)} & \textbf{Depth} & \textbf{Multi-head Attention} & \textbf{English} & \textbf{Russian} & \textbf{$\Delta$}\\ 
\midrule
138.69 & 1 & 12  & 66.6 & 45.0 & 21.6 \\
136.32 & 2 & 12 & 73.7 & 55.7  & 18.0 \\
136.20 & 4 & 12 & 76.9 & 59.0  & 17.9 \\
138.86 & 6 & 12 & 78.3 & 63.1  & 15.2\\
134.00 & 8 & 12 & 78.6 & 62.3  & 16.3 \\
\midrule
132.78 & 12 & 12 & 0.790  &  0.657  & 0.133 \\
\bottomrule
\end{tabular}
    \begin{tablenotes}
    \small
    \item Number of multihead attention and total number of parameters are fixed. (size of hidden units and intermediate units are changed so that total number of parameters remains almost same)
    \end{tablenotes}
\end{threeparttable}
}
\parbox{.45\linewidth}{
\small
\centering
\begin{threeparttable}
\caption{Model Architecture - Contribution of Multi-head Attention }
\label{tbl:multiheadAttention}
\begin{tabular}{ c c c c c c} 
\toprule
\multicolumn{3}{c}{} & \multicolumn{3}{c}{\textbf{XNLI}} \\
\cmidrule{4-6}
\textbf{Parameters (in Millions)} & \textbf{Depth} & \textbf{Multi-head Attention} & \textbf{English} & \textbf{Russian} & \textbf{$\Delta$}\\ 
\midrule
132.78 & 12 & 1 & 77.4 & 63.2 & 14.2 \\
132.78 & 12 & 2 & 78.3 & 62.8 & 15.5 \\
132.78 & 12 & 3 & 79.5 & 65.3 & 14.2 \\
132.78 & 12 & 6 & 78.9 & 66.7 & 12.2 \\
\midrule 
132.78 & 12 & 12 & 79.0  &  65.7  & 13.3 \\
\bottomrule
\end{tabular}
    \begin{tablenotes}
    \small
    \item Depth and the total number of parameters are fixed. Number of parameters are function of Depth, hidden size and Intermediate size.
    \end{tablenotes}
\end{threeparttable}
}
\end{table*}

\subsubsection{Number of Attention Heads}

In this section, we study the effect of multi-head self-attention on the cross-lingual ability of bilingual BERT. We fix the depth and the total number of parameters -- which is a function of depth and size of hidden and intermediate units. From Table~\ref{tbl:multiheadAttention}, we can see that the number of attention heads does have a significant effect on cross-lingual ability($\Delta$). Bilingual BERT is satisfactorily cross-lingual even with a single attention head. \swm{nice results. there was some recent work that studied this. can we cite them?} \kk{Need to read the paper}



\subsubsection{Total Number of Parameters}
Similar to the depth we also anticipate that a large number of parameters could potentially help BERT extract good semantic and structural features. We study the effect of the total number of parameters on both monolingual and cross-lingual performance by fixing the number of attention heads and depth we change the number of parameters by changing the size of hidden and intermediate units (size of intermediate units is always 4$\times$ size of hidden units).

From Table~\ref{tbl:NumberOfParameters}, we can see that total number of parameters are not significant after a threshold, however it is significant until a threshold, which suggests that bilingual BERT requires a certain minimum number parameters to extract good semantic and structural feature. We expect this threshold to be larger when the model is trained with more data or many languages.  \kk{This paragraph needs to changes according to results.}



\begin{table*}[!htbp]
\small
\centering
\begin{threeparttable}
\caption{Model Architecture - Contribution of Total number of Parameters}
\label{tbl:NumberOfParameters}
\begin{tabular}{ c c c c c c} 
\toprule
\multicolumn{3}{c}{} & \multicolumn{3}{c}{\textbf{XNLI}}\\
\cmidrule{4-6}
\textbf{Parameters (in Millions)} & \textbf{Depth} & \textbf{Multi-head Attention} & \textbf{English} & \textbf{Russian} & \textbf{$\Delta$}\\ 
\midrule 
7.87 & 3 & 3  & 0.685 & 0.432 & 0.253 \\
12.19 & 3 & 3 & 0.701 & 0.441 & 0.260 \\
16.78 & 3 & 3 & 0.708 & 0.504 & 0.204 \\
\midrule 
8.40 & 6 & 6 &0.702 & 0.497 & 0.205\\
13.37 & 6 & 6 &0.724 & 0.562 & 0.162 \\
18.87 & 6 & 6 & 0.733 & 0.544 &  0.189 \\
\midrule
29.65 & 12 & 12  &  0.766 &  0.614 &  0.152 \\
44.89 & 12 & 12  & 0.782 & 0.640 & 0.142 \\
89.03 & 12 & 12  & 0.786 & 0.641 & 0.145 \\
192.86 & 12 & 12  & 0.788 & 0.669 &  0.119\\
283.11 & 12 & 12  & 0.796 & 0.654 & 0.142 \\
\midrule 
132.78 & 12 & 12 &0.790  &  0.657  & 0.133 \\
\midrule
\bottomrule
\end{tabular}
    \begin{tablenotes}
    \small
    \item Depth and number of attention heads are fixed. Total number of parameters are varied by changing hidden size and intermediate size.
    \end{tablenotes}
\end{threeparttable}

\end{table*}



==> OldRelatedWorks.tex <==
% \citep{wu2019beto} has studied the cross-lingual ability of multilingual BERT on different semantic and syntactic tasks. 

\citep{wu2019beto} shows the multilingual BERT proposed by~\cite{devlin2018multi} is surprisingly cross-lingual and provides comprehensive experiments on 5 different tasks and 38 different languages to verify the cross-lingual ability of multilingual BERT. \citep{wu2019beto} fixes the multilingual BERT and studies the characteristics of features extracted at different layers, they also show that multilingual BERT benefits from shared wordpieces between train and test set.

\citep{pires2019multilingual} shows that multilingual BERT generalizes across languages with different scripts further they use code-switching and transliteration to show that multilingual BERT doesn't generalize to languages it was not pre-trained on

% XLM~\citep{lample2019cross} proposes the Translation Language Modeling (TLM) objective to improve cross-lingual performance by leveraging parallel data when available

XLM~\citep{lample2019cross} improves the cross-lingual performance of multilingual BERT by incorporating knowledge from parallel data using a new learning objective --  Translation Language Modeling (TLM). 


\dr{Integrate to two coherent paragraphs: the first two papers, as a study of mBERT -- distinguish from the type of analysis we do; then the XLM and the multi-head papers: discuss what they do, and show that we deal with additional issues and explain some of their findings (the XLM paper).
This need to move to be the paragraph before  the contribution in the Introduction.}

==> oldIntroduction.tex <==
%% Use NewIntroduction.tex

% % What is the problem statement. Why do we care
% Unsupervised language representations, paired up with sufficient supervised training data, have been ubiquitous in most English NLP tasks. For other languages, especially, low resource languages, where it is hard or expensive to collect sufficient training data, cross-lingual models have been developed to transfer knowledge from high resource languages to low resource ones. 

% Multilingual BERT\footnote{https://github.com/google-research/bert/blob/master/multilingual.md.}, a Transformer-based \citep{vaswani2017attention} language representation model trained on the unsupervised text of 104 languages together with a language modeling objectives (Masked Language Model and Next Sentence Prediction) provides a representation that is generalizable across languages for a variety of downstream tasks, despite being trained with no explicit cross-lingual objective. In light of previous works ~\citep{conneau2017word,faruqui2014improving,luong2015bilingual} that strive hard to explicitly model cross-lingual relationships, this simple model is intriguing. 

% % What is known: success in literature.

% Recent work~\citep{wu2019beto,pires2019multilingual} has shown multilingual BERT (mBERT) is surprisingly cross-lingual and studied the zero-shot/cross-lingual performance on a variety of tasks and languages pairs (Train-Test language pairs). XLM~\citep{lample2019cross} proposes the Translation Language Modeling (TLM) objective to improve cross-lingual performance by leveraging parallel data when available. \citep{wu2019beto} shows that fixing the bottom layers of multilingual BERT during fine-tuning further improves the performance of BERT, it also observes a strong correlation between the extent of word-piece overlap between the train and test data during the \textit{fine-tuning} and cross-lingual performance. \citep{pires2019multilingual} hypothesize that shared word-pieces forces multilingual BERT to learn generalized representation. \kk{@Dan if you think this paragraph is not required then we can remove it -- I thought it gives some flow for what is the currently lacking}

% While the current literature focuses on improving the cross-lingual performance and analyzing the multilingual BERT for various scenarios by considering it as a \textit{black box}, there has been no systematic study on the most intriguing parts: \textit{What makes multilingual BERT cross-lingual? What components of multilingual BERT affects the cross-lingual ability?} In this work, we fill this void by providing a systematic empirical study on various components of multilingual BERT using two conceptually different tasks -- cross-lingual Textual Entailment and cross-lingual Named Entity Recognition -- and three different languages -- Spanish, Hindi, and Russian, along with English. 

% We analyze multilingual BERT in three orthogonal dimensions
% \begin{enumerate*}
%     \item Linguistics
%     \item Architecture
%     \item Input and Learning Objective.
% \end{enumerate*}
% \drc{In all cases, we study the mBERT model in the context of two languages, English, and a second language. To avoid confusion, we will call this model from now on bBERT.} 

% In the Linguistics, we study the contribution of
% \begin{enumerate*}[label=(\roman*)]
%     \item word-piece overlap, and
%     \item structural similarity 
% \end{enumerate*}
% between the source and target languages. Contrary to the current hypothesis~\citep{pires2019multilingual}, our results show that \textit{multilingual BERT is cross-lingual even when there is absolutely no word-piece overlap}. Interestingly the cross-lingual performance is not affected much by word-piece overlap. Our results also suggests that structural similarity(\ref{subsec:Structure}) is much more important.

% As a part of Architecture, we study the importance of
% \begin{enumerate*}[label=(\roman*)]
%     \item depth 
%     \item multi-head attention, and
%     \item total number of parameters in multilingual BERT.
% \end{enumerate*}
% Our results suggest that the depth and the total number of parameters of multilingual BERT are crucial for both monolingual as well as cross-lingual performance, whereas the multi-head attention is not very significant -- even with single attention head multilingual BERT gives satisfactory results. 

% In Input and Learning Objective, we study the effect of 
% \begin{enumerate*}[label=(\roman*)]
%     \item next sentence prediction (NSP) objective,
%     \item language identity marker in input, and
%     \item character vs word-piece vs word tokenization
% \end{enumerate*}. 
% Our results show that the next sentence prediction objective hurts cross-lingual performance. Multilingual BERT~\citep{devlin2018multi} says that they don't use any language identity marker so that multilingual BERT can work in a zero-shot way, however, our results suggest that multilingual BERT is cross-lingual even if we add a language identity marker. Our experiments also show that character tokenized BERT performs significantly worse than word-piece tokenized BERT. 

% Current analysis on multilingual BERT~\citep{pires2019multilingual, wu2019beto} \textit{fixes} the pre-trained multilingual BERT and studies its cross-lingual effectiveness at different layers and different fine-tuning scenarios, like effect of word-piece overlap during fine-tuning, differences in word-ordering (SVO/SOV) between source and target language. In contrast, we change the pre-training part of multilingual BERT in a controlled way and study the effect of different components for its cross-lingual ability as multilingual BERT attains its cross-lingual ability from pre-training -- even agreed by ~\citep{pires2019multilingual}.

% Several works~\citep{liu2019roberta,yang2019xlnet, joshi2019spanbert} question the necessity of NSP objective and shows that it might actually hurt the performance of monolingual BERT, in this work we study the effect of NSP objective on cross-lingual ability. \citep{lample2019cross} shows that XLM, which doesn't use NSP objective, outperforms multilingual BERT, however they don't provide a fair comparison (many other components change -- architecture, number of languages, etc..) to study the effect of NSP in isolation, we complete the void by providing a controlled and fair comparison. \citep{voita2019analyzing, clark2019does} provides a probing study on the multi-head attention of transformer models and shows that most attention heads are redundant; in this work we study the effect of multi-head attention for cross-lingual performance of multilingual BERT. The key contributions of our work are as follows:
% \begin{itemize}[nosep]
%     \item We are the first to provide a systematic study on the cross-lingual ability of multilingual BERT. 
%     \item We provide a novel approach to study word-piece overlap in a controlled way. 
%     \item Many interesting findings -- multi-head attention and wordpiece overlap is not significant; structural similarity, depth, and number of parameters of multilingual BERT are crucial.
% \end{itemize}

% % \kk{Key contribution needs more editing}\dr{Contributions: (i) 1st multilingual analysis of mBERT. (ii) A methodology for a multilingual analysishttps://www.overleaf.com/project/5d7700da03e20d0001325858 (fake English). (iii) key results. }












% % \swm{key contributions would be good. other advice: don't worry about space right now. It's easy to cut material later, much much harder to add content that's missing.}


% % \begin{itemize}
% %     \item We show that multilingual BERT is cross-lingual even when there is no word-piece overlap. 
% %     \item We show that Structural similarity is more important
% %     \item We show that depth and number of parameters are crucial, and multihead attention is not very significant for cross-lingual performance.
% %     \item Next sentence prediction hurts cross-lingual performance 
% %     \item Word-piece based BERT is significantly better than character based BERT.
% %     \item Adding language identity marker doesn't affect cross-lingual ability of BERT.
% % \end{itemize}




% % We provided extensive experiments on three language pairs, English - Spanish, English - Russian, and English - Hindi, where the second language vary in different scripts and typological features. We evaluate performance of \BBERT on two downstream tasks, cross-lingual Textual Entailment and cross-lingual Named Entity Recognition.

% %We also compare cross-lingual similarity of multilingual BERT with multilingual flair and multilingual word2vec. 
% %Our key contribution is, we isolate and provide systematic study of multilingual BERT. 









